Navigating Conceptual Space; A new take on Artificial General Intelligence

Edward C. Tolman found reinforcement learning unsatisfactory for explaining intelligence and proposed a clear distinction between learning and behavior. Tolman's ideas on latent learning and cognitive maps eventually led to what is now known as conceptual space, a geometric representation where concepts and ideas can form points or shapes.Active navigation between ideas - reasoning - can be expressed directly as purposive navigation in conceptual space. Assimilating the theory of conceptual space from modern neuroscience, we propose autonomous navigation as a valid approach for emulated cognition. However, achieving autonomous navigation in high-dimensional Euclidean spaces is not trivial in technology. In this work, we explore whether neoRL navigation is up for the task; adopting Kaelbling's concerns for efficient robot navigation, we test whether the neoRL approach is general across navigational modalities, compositional across considerations of experience, and effective when learning in multiple Euclidean dimensions. We find neoRL learning to be more resemblant of biological learning than of RL in AI, and propose neoRL navigation of conceptual space as a plausible new path toward emulated cognition.

==> neoRL.tex <==
\section{Decision agents by disributed RL over NRES} %{Experiment: Situation-Attributed Traits as objectives for distributed aspects of navigation}
%{{{ IKKJE EN DEL AV ARTIKKELEN
\label{sec:neoRL}
    We now turn our attention back to NRES and considerations related to forming decision agents by a distributed SAT space.
    % We now turn our attention back to NRES and how to accomplish autonomous navigation in tech.
    % TODO Skrive om leddsetninga! TODO
    % Assuming that problem representation reflects how the system approaches the problem, we praise the mechanisms for NRES as the best insight into how to accomplish navigational autonomy.
    %Assuming that the solution is formed by problem representation, mechanisms for NRES can very well be our best source of inspiration for navigational autonomy.
    %%%%%%%%a             %%%%%%%%              %%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Take for example the place cell modality from our sense of orientation:
    For a set of features composed of mutually exclusive receptive fields, each NRES modality could form a set of independent scalar reward signals for creating separate value functions based on SAT.
    % From a set of features composed with mutually exclusive receptive fields, this group of SAT could form the orthogonal scalar signals required for singular value components of the value function.
    A simple set of features with comprehensive coverage is illustrated in Figure \ref{fig:bluedot_with_target}.
    Each SAT in this NRES map now provides a scalar measure of success related to the desire for accomplishing the corresponding NRES cell.
    Singular Value-function Components (SVC) can be learned as the value function for instinctual desires toward the individual SAT. % of this NRES modality.
    % Singular Value-function Learners (SVC) can now learn the value function connected with instinctual desires only concerned with accomplishing this SAT. % and toward this SAT.
    % % Singular value learners can now form the value function related to this desire.
    %     %learners that are concerned only with how to achieve one SAT learns a value function with regard to the corresponding objective.
    % The full set of SVC can now be thought of as uncoordinated instinctual desires with respect to agent behaviour.
    % % The set of learners now represent an uncoordinated set of instinctual desires.
    With analogies to Freud's structural model of the psyche, SVC could also be thought of as a product of \emph{Id} --- an instinctual aspect of the agent that only seeks pleasure\footnote{
    %With analogies to Freud's structural model of the psyche, the individual learner can be thought of as an \emph{Id} of the agent psycho, a part of the unconscious that only seeks pleasure\footnote{ 
        Freud's Id agency of the human psyche is governed by uncoordinated reward-driven impulses analogue to the reward hypothesis.} \cite{freud1940outline}.
        %In some ways similar to the hedonistic aspect of the RL reward hypothesis} \cite{freud1940outline}.
    Directed effort can emerge through an organizing higher mechanism of the psyche. %, combining interests and prioritizing and aggregating desired originating from Id.
    %Directed effort only emerge through organizing higher mechanisms of the psyche, combining interests and aggregating the desire originating from Id.
    Similarly, behaviour synthesis by series expansion of orthogonal SVC is believed to allow for a distributed state representation in \mbox{NRES-Oriented RL}.
    % Behaviour synthesis by series expansion of orthogonal SVC is believed to allow for distributed state representations as found in NRES for autonomy.
    % Learning value functions for instinctual desires is relevant when considering distributed RL.
    %%
    % TODO AVSLUTT PAGARAPH TODO 
    %  Through distributed learning 
    %Via a clear separation of the learning aspect and the acting aspect of an agent, the learning agent can further be divided into fundamental desires;
    %fundamental desires by SVC can further be combined though series expansion.
    
        % it is possible to learn instinctual desires, uncoordinated value functions toward different aspects of the environment.
    %Only by higher order mechanisms can directed effort arise. % as a balance between 

%    %   given a set of features with mutually exclusive receptive fields, each of the SAT of this NRES set could be considered a state in a restricted MDP.
%    % A simple feature set with comprehensive coverage in 2D is demonstrated in figure \ref{fig:bluedot_with_target}. %: a set of artificial NRES feature detectors cover the whole Euclidean plane.
%    Any feature in such a state set could be considered as the objective of an agent, only concerned with the activation signal of the corresponding SAT.
%    With the sole interest of activating one particular feature, with an activation signal given by that feature's SAT, this basal agent component can learn the state-action value with regards to activating that feature.
%    %The activation of feature $[4,4]$ in figure \ref{fig:bluedot_with_target} would cause a reward signal $\mathbb{R}=+1$ to the basal learner associated with feature $[4,4]$ and $\mathbb{R}=0.0$ to every other in this set.
%    %%%%%%%%%%%%%
%    With the capability of learning off-policy, this particular agent could be considered as one GVF-inspired \emph{learner}, only concerned with learning the value function with regard to the corresponding scalar activation signal.
%    With capabilities of learning a value function irrespectively of the agent decision process, it is possible to have one learner associated with every feature of the NRES set.
%    % For each feature in this set, let there be one GVF-inspired \emph{learner}, only concerned with the scalar activation signal SAT.
%    With analogies to Freud's structural model of the psyche, we refer to this instinctual learner as an \emph{Id} of the agent entity;
%        the full set of Ids represent an uncoordinated set of desires toward selecting different actions based on the current situation.
%    Only through an organizing structure, the ego, can directed effort arise.


    %%%%%%%%%%%%%%
    %Having the role of an instinctual uncoordinated desire, this auxiliary value function learner could be thought of as a digital variant of Freudian \emph{Ids} \footnote{From Freud's structural model of the human psyche.}.
    %Higher-order structures for organizing behaviour, the \emph{ego} in the agent structure, could for very simple tasks be defined by constant priorities.
    %.. to point out how navigation in abstract conceptual spaces have been proposed as a mechanism behind reasoning and thinking \cite{bellmund2018navigating}.
    %We maintain our focus on NRES for navigation in this article, and define the organizational aspect of the decision agent apparatus to be formed by a priority defined by the reward received when navigating to one object of interest.
    %%     Directed effort by an autonomous agent would have to be organized by a higher aspect of our decision agent, possible to learn by similar mechanisms.
    %Through Bolzmann addition for incorporating priority and Bolzmann summation for integrating all considerations into the policy-generating value function, we see how this structure allows for superposition in the value space.

    % In this section we will limit our focus to exploring whether such an approach is plausible, and to which degree the Id is a plausible approach for cybernetic autonomy.


    \begin{figure}[th!bp]
        \centering
        \fbox{\includegraphics[width=0.7\columnwidth]{figures/bluedot_N5_with_target}}
        \caption{   \small
            A $N5$ one-hot simplification of NRES.
            This computationally trivial mapping illustrates how SAT receptive fields could form a comprehensive mapping by receptive fields. % by dividing the Euclidean space into $N^2$ same-sized receptive fields.
            With each axis of the Cartesian representation of the plane divided into $N = 5$ equal intervals, we refer to this as a $N5$ representation of this plane.
            Although not plausible in biology, this simplification can help clarify further argumentation and understanding. %; the biologically plausible hexagonal pattern is believed to give better results.
            Individual MDPs can be constructed for the SAT of each tile, as presented for the SAT $[4,4]$ above.
            % The simplest possible 
            % More biologically plausible mappings are believed to give better results, e.g. by the hexagonal pattern often found in NRES.
        }
        \label{fig:bluedot_with_target}
    \end{figure}


    % <bygge opp eit RL problem av eit SAT sett; korleis en ny repr. kan gi eit nytt MDP>
    Forming instinctual desires by RL over a distributed SAT representation requires some consideration with respect to the Markov property.
    % I have identified two important considerations for decomposing the prediction problem.
    %       |1|
    Firstly, Euclidean space must be represented by a finite set of unique states to form an MDP.
    This aspect is well handled by the NRES faculty for discretization, combined with the requirement of only considering mutually exclusive SAT.
    %This discretization can for example be achieved by NRES feature detectors being mutually exclusive; % as presented in \ref{sec:one-hot}.
    % This discretization can very well be handled by the NRES feature detectors as presented in \ref{sec:one-hot}.
    %    one-hot encoding is a convenient way for creating a unique mapping between Euclidean space and the activation pattern of NRES states.
    % The map between Euclidean space and a discrete set of NRES states have to be unique, something that is simplest to accomplish by requiring the SAT receptive fields to be mutually exclusive.
    %       |2|
    Secondly, the set of choices available must be such that any state combined with any choice uniquely defines the probability distribution for the next state. 
    As the state set already is defined by NRES SAT, the Markov property must be fulfilled through careful consideration of when state update occurs.
    % The state set for concurrent MDPs of NRES is fixed to this representation, and the Markov property must be fulfilled by consideration of when state update occurs.
    % %The state set for concurrent MDPs of NRES is fixed to the distributed SAT representation, as mentioned above.
    % The Markov property have to be fulfilled from unconventional considerations, and necessitating a revisit to the intentions behind the Markov property.
    % % In order to fulfill the Markov property, allowing to consider the individual learning challenge under the RL framework, we need to revisit the intentions behind the Markov property.
    At the \emph{time} of state change, the state is updated according to the probability distribution defined by state and action \cite{bellman1957markov}.
    % % VELDIG BRA, men TOO MUCH: Utsette dette til en egen artikkel:
    In board games and early RL environments, time can be defined as a sequence that iterates after action selection:
        % TODO skrive om att neste setning! TODO
        A direct link between action selection and state development allows the presumed {cause} to be considered as what drives learning. %causality.
        %Due to a direct link between action selection and time increment in traditional RL environments, the presumed {cause} could be considered as what drives learning.
    % Allowing self-transitions for the Markov state, this mechanism could be extended temporally trivial board games.
    By allowing self-transitions in the state set, the validity of \emph{action-driven learning} is extended beyond temporally trivial board games.
    % By allowing self-transitions for the Markov state, the validity of actions as {learning driver} is extended beyond temporally simple board games.
    For slightly more interesting temporal progression, traditional action-driven learning could prove to be challenging for state-of-the-art RL methods \cite{machado2018revisiting}.
    % For slightly more interesting temporal progression, traditional action-driven learning could introduce some interesting challenges for state of the art RL methods \cite{machado2018revisiting}.
    % For slightly more complicated temporal progression, this introduces challenges \cite{machado2018revisiting} that requires stochastic function approximation.
    % This could introduce some fundamental challenges for simple systems, but within what is possible to handle by stochastic methods or AI function approximation \cite{machado2018revisiting}.
    For physical systems, however, where temporal progression could be fully disconnected from the agent's decision, 
        considering a predefined set of actions as what drives learning imposes strict limitations to the temporal scope of what is learned. %as defined by this set.
        %action-driven learning forces us to pre-define the set of actions, and consequently the temporal scope of the agent. 
    % For physical systems, however, with potentially zero connection between temporal progression and the agent's decision, action-driven learning can be damaging to agent performance. 
        %%it is hight time to revisit our understanding of causality.
    For NRES-Oriented RL, with a fundamental focus on the environment and intended for the real-world, a more appropriate driver for learning might be {the effect} of the causal relation: 
            %it is more appropriate to focus on {the effect} in causal relations:
    % In NRES-Oriented RL, intended for interaction with the real-world, it could be more appropriate to focus on {the effect} in causality: % it could be better to focus on {the effect} as what drives learning:
    Triggering a Markov update after state change rather than after every presumed cause of such, \emph{effect-driven} learning could allow for MDPs to be defined for each SAT in NRES.
        %--- learning the value of any considered action with regard to that objective. 
        % could very well be more temporally robust.
    % By letting the Markov update happen after state change rather than after every presumed cause of environmental change, 
    %     \emph{effect-driven} learning could very well be more effective and temporally robust for complex environments.
    % % % Kort ned på neste setninga: Bra setning ellers! TODO
    % Instinctual desires as expressed by SVC can now be learned in isolation without the need for pre-defined action sets or constrained temporal extent. 
    % Instinctual desires can now be learned separately and simultaneously for every single SVC without ever needing to define or limit the action set. %the need to define the action set à priori.

    %For NRES-Oriented RL, this situation could be ameliorated by instead focusing on hte  perhaps better approach would be to instead 
    %For NRES-Oriented RL, a perhaps better approach would be to focus on {the effect} as learning driver for inference learning.
    % % With cause and effect both being valid candidates for interaction learning, a perhaps better approach for temporally robust inference learning could be to focus on \emph{effect} as learning driver.
    % % % A perhaps better approach for temporally robust inference learning would be to focus on the \emph{effect} as learning driver;
    % % % With cause and affect both being valid candidates for learning about inferences, NRES-Oriented RL could be effect-driven.

    %%%%% GODSAKER TIL DISKURS?
    %By result-oriented inference learning, instinctual desires based on NRES can be learned by each learner by pure observation and pure off-policy learning.
    % A perhaps better approach for temporally robust inference learning would be to focus on the \emph{effect} as learning driver;
    %    when learning happens as a result of state transition rather than after every instance of possible causes of such, learning is a result of changes in the environment rather than happening after every basal action selection.
%    A perhaps more suitable approach for NRES-oriented RL is to consider the \emph{effect} as the learning driver.
        %focusing on the causality rather than when transition is supposed to occur.
    %With learning after the effect rather than our presumptions of possible causes, inference learning becomes temporally robust and ready to handle real-world situations.
    % When learning happens as a result environment state change rather than our presumptions on possible causes, effect-driven inference learning becomes more temporally robust to handle real-world situations.
    %
    % Learning what caused the state change is more temporally robust as such learning does not have to consider action set granularity to account for multiple time scales.
    %%%%%%%%%%%%
    %     For physical systems, however, connecting basal actions with temporal propagation in the environment makes little sense. % and only imposes requirements as to when state transition is supposed to occur.
    % % For physical systems, however, linking basal action selection with the temporal aspect of causality imposes too strict requirements as to when state transition occurs.
    % Temporal progression in the real world does not adhere to deterministically simple rules as found in board-games or other traditional RL environments. %, computer simulations, or some algorithmic challenges. 
    %%%
    % TODO SKRIVE NESTE SETNING PÅ NY:    [litt lett setning om 2 sider ved causality]
    % Since both sides of causal relationships, cause and effect, are candidates for what drives learning, NRES-Oriented RL could consider \emph{effect} to be the learning driver.
    % %  Both sides of causality, cause and effect, are candidates for what drives learning.
    % % NRES-Oriented RL requires \emph{effect} to be the learning driver;
    %%
    % In effect-driven learning, the Markov update happens after state change rather than after presumed causes of environment change.
    % A positive side effect is that inference learning becomes temporally robust, focused on environmental effects, and inference learning becomes temporally robust and ready to handle real-world situations.


    %With learning happening as a result of state transition instead of possible causes of such, inference learning becomes less oriented around absolute time or by action granularity.
%    % Learning will now happen as a result of state transition instead of action of time since possible causes, allowing for inferences that are less oriented to absolute time spam between cause and effect.
%    %If we define learning to happen as a result of state transition rather than any possible cause, this would make inference temporally robust.
%    %In effect-driven learning, learning happens as a result of state transition rather than possible causes of such.
    % This result-oriented variant of inference learning now allows for learning what actions caused the transition rather than learning the effect of each option.
    %%%

    % The difference is as subtle as its implications are grand. % and but the implications 
    % By result-oriented inference learning is is possible to learn instinctual desires based on observation and pure off-policy learning.
    %State sets defined by NRES feature detectors can now learn by observation and pure off-policy learning.

    %     With learning happening after \emph{the effect} rather than \emph{the cause} of a causal relationship, off-policy learning is result-oriented rather than focusing on own actions.  %becomes more effective.


    %%%
    %     with action as a learning driver -- deciding when the Bellman update is performed -- the granularity of action set will also define \emph{when} the agent learns. %have a major impact on when the agent learns.
    % This defining aspect of learning thus probhibits changes in action space after learning starts. %makes it impossible to change the action space during execution.
    % %%
    % Consider instead to have SAT transitions as learning driver in our NRES SAT space:
    %     With learning happening after \emph{the effect} rather than \emph{the cause} of a causal relationship, off-policy learning is result-oriented rather than focusing on own actions.  %becomes more effective.
    % % TODO Neste setning henger ikkje heilt sammen TODO
    % After every SAT transition, when the state of the NRES representation is updated, this is when it becomes pertinent to learn what caused the transition.
    % For state sets defined by NRES feature detectors, a transition-based learning driver allows for MDPs with true off-policy inference learning. % by pure observation.

    %Causality can be defined from the cause, i.e. what will be the effect ($s \to s'$) of performing $a$ from state $s$.
    %It is also possible to consider causality by the effect, i.e. after transition $s \to s'$, what was the probable cause $a$ of this transition?
    %The subtle difference is when learning happens.

    %% Secondly, the choices available for the next action selection by the agent must be such that any state combined with any action uniquely determines the probability distribution for the next state.
    %The Markov property is a fundamental requirement for MDPs, is often seen as an attribute of state representation\footnote{
    %                The RL literature generally refers to this as being a property of state, under the name Markov state.}
    %%The Markov property is a fundamental requirement for MDPs, and is often seen as an attribute of state representation 
    %%                \footnote{In the RL literature it is possible to find references to the Markov property as an attribute of the state, e.g. by the name ``Markov State'' \cite{sutton2018reinforcement}.}.


    % This property is often seen as an attribute of the state \footnote{The reference work in RL sometimes refers to the Markov Property by the name ``Markov State'' \cite{sutton2018reinforcement}.}.
    % It is important, however, to remember that the Markov property is a product of state and action after action selection in an MDP \cite{bellman1957markov}; %a defining requirement for actions of an MDP.
    
    %%
    %% % It is important that it is the combination of state and possible choices, giving the probability distribution for the next system state, that together satisfy the Markov property.
    %% Further, as learning in RL happens after every action, defining the granularity of what is learned, \emph{actions as learning driver} will have major impact on the trained agent. %of this MDP.
    %% % After the cause, we learn from the effect of this cause, defining the action as the main driver for learning.
    %% %It is, of course, possible to turn this around and focus on the effect in the causality;
    %% We could, of course, turn this around focus on the effect of the causality instead; 
    %%    % and rather focus on the inferred result; %instead consider the causal result as what drives learning; %as the learning driver for NRES-oriented RL approaches:
    %%    In the NRES-oriented state space representation of a complex and generally unobservable system, it makes sense to define causality by the result rather than by considering every possible cause.
    % In particular for NRES feature detection as the state space of the MDP, a transition-based learning driver allows for true off-policy inference learning.
    %%
    % Til diskurs: 
    %| Given an MDP defined by this state set and by all possible transitions, {N, E, S, W}, the resulting representation would form an MDP with transition probability 1.
    %| Also known under the name Finite-State Machine, this representation combined with RL could very well be a first step toward autonomy. [NÅKKA].
    %%%%%%%%%%%%%%%
    %The resulting environment representation, defined by the NRES state space with the learning driver defined by transitions in this set, allows for defining separate MDPs for each receptive field in the NRES;
    %    with SAT activation as the reward signal for each of the possible sub-MDPs, learning instinctual desires can happen from pure observation.



        
\subsection{A Simple Navigation Experiment: WaterWorld} % WW with a single creep.
    \label{sec:experiment}
    % Since we compose behaviour by superposition principles over the desires from weighted instincutal learnes, it would be possible to take inspiration from a gread body of techniques from other branches of machine learning.
    A simple but realistic environment for navigation can be found in the PyGame allocentric implementation of Karpathy's WaterWorld \cite{webWaterWorld_in_PLE}.
    The task is to catch a floating object in a continuous plane.
    % The task is to catch a floating object in a continuous environment with inertia mechanics. %where basal actions control one's acceleration.
    This challenge is an example of how difficult an environment governed by basic physical laws can be for RL;
    %This simple challenge in an environment governed by basic physical laws exemplifies how difficult learning can be for physical systems;
        the WaterWorld challenge is listed as an unsolved challenge by AI by OpenAI \cite{webWaterWorldUnsolved_openai}.
    The navigational state being represented in an allocentric Euclidean plane representing the position of the agent and the position of the object of interest.
    Whenever the agent touches the object, a reward of $+1$ is given, and the object is re-spawned with a random location and speed vector.





    % No previous knowledge or function approximation  ... anna enn det som er beskrevet i denne teksten.
    % No previous knowledge or precursor exist other than the design as presented in this text.

    \begin{figure*}[tb]
        \centering
        \includegraphics[width=0.95\textwidth]{figures/10-40_svart_control_vartiant2}
        \caption{     \small
            Transient proficiency of a number of neoRL agents in the allocentric WaterWorld challenge with a single object of interest;
            neoRL proficiency at the task is measured as received reward per second.
            Due to the sparse nature of the challenge, a per-timestep average is taken across $100$ individual runs for each curve.
            The control in black shows the performance at the task for random actions with no learning. 
            The agent and the object of interest have a random encounter on average every 7-8 seconds.
            Low NRES resolutions, $N5 - N15$ are comparable with the control, indicating that NRES of low resolution does not improve performance.
            From NRES resolution $N20$, every step in NRES resolution results in significantly better neoRL performance.
            % At $N40$, with 1600 allocentric SAT, one would expect learning to happen much slower than e.g. $N25$, with 625 SAT 
            Noisy data with sparse rewards forces us to 
            As can be seen from the control, data is
            % TODO Skriv at 50K var nytta, men at uttrekk er gjort; læringa var så effektiv at kurva fortsetter uten endring etter 20K.
        }
        \label{fig:experiment_results}
    \end{figure*}

    
    %<KORLEIS AGENTEN FUNKER>
    The agent is governed by SVCs as defined by a place-cell NRES modality, with a resolution from $N5$ to $N40$ according to the formalism illustrated in figure \ref{fig:bluedot_with_target}.
    %The agent is implemented with a place-cell NRES modality, with a resolution reported as the discretization along each axis as seen in figure \ref{fig:bluedot_with_target}.
    %%
    With the value function of the agent being the weighted sum over all instinctual learners, the behaviour is defined by how much we let each SVC affect agent value function. % to the value function of the individual learner. 
            %the control imposed by changing the priority for each allows for a higher level of abstraction.
    % The most basic approach would be to let the contribution from each GVF be scaled by the estimated reward of achieving the corresponding SAT.
    With a single object of interest worth a constant reward, the priority-defining abstraction layer reduces to only activating the learner associated with containing SAT. 
        %can be simplified into activating the learner associated with the SAT that contains this object.
    % For an experiment with a single object of interest, the higher level of abstraction reverts into simply activating the policy toward the SAT containing the desired object;
    The learner associated with the object has a priority (weight) corresponding to the object's reward. 
    All other learners have a priority of $0$.
    Behaviour is formed based on a weighted sum over relevant considerations' value function. % defines the value function of the agent. 
        %aggregate value function defines priorities affects how much we listen to different instinctual desired 
    %Policy is formed based on the weighted sum over all relevant considerations.
    % With a single object of interest, only the GVF corresponding to the SAT containing the object have a positive scaling.

    % <korleis plotta lagast>
    % The proficiency of the agent can be measured by the how much reward is received at any moment in time.
    % Starting out with zero knowledge of the task or environment, the agent learns in real-time. % during the experiment time course of 1000 seconds.

    % skrive om 50K !!!
    The agent has zero knowledge of the task at the beginning of each experiment.
    Learning happens in real-time, with the continuous flow of experience being the only basis for learning.
    A single run with 50K time iterations takes just under 1000 seconds on a sufficiently strong computer.
    % When the experiment is throttled by high system load, this affects the simulation as well as agent computation; within the simulation, learning is still performed real-time with the simulation.
    Due to the sparse measure of success, where the agent only receives $\mathbb{R}$ when the object is captured, 100 separate runs have been performed to present the per-timestep average.
    The curves have been further processed by a first-order Butterworth low-pass filter.


    In Figure \ref{fig:experiment_results} the first 20K time steps can be seen; due to high learning efficiency, we have zoomed in on the first half where learning happens.
    %Due to the learning efficiency demonstrated by the NRES-Oriented agent, Figure \ref{fig:experiment_results} have zoomed in on the first 20K time steps. %it was deemed redundant to show the full 50K experiment length.
    The demonstrated learning efficiency indicates that this task might be too simple for displaying the potential of neoRL.
    Still, for the sake of clarity and keeping a singular focus, the initial experiment is presented; this work is a conceptual plausibility study, and clarity for the experiment is more important than complexity.
    The agent rapidly reaches final proficiency at the task, limited by NRES resolution.

    % With a desire to find the time course of agent proficiency, an average over 100 individual runs 
    % Interested in the transient time course for agent proficiency, it was necessary to average over many individual runs.
    Each curve is based on data from 100 individual runs, where the environment and agent are completely restarted for each run.
    % Still, due to the sparse measure of success, only receiving $\mathbb{R}$ when the object is captures, a first-order Butterworth low-pass filter have been applied to make data presentable.
    With control in black represent Brownian motion, i.e. $\epsilon$--random walk policy, we can see that $N5-N15$ NRES resolution does not improve agent proficiency for this problem setting.
    From $N20$, however, we can see a steady increase in agent performance with increasing NRES resolution for the neoRL agent.
    %%
    %We can also see how the agent learns to perform this simple task in a matter of minutes, reaching final proficiency as defined by SAT receptive fields.
     We can also see how the agent learns to perform this simple task in a matter of minutes, reaching final proficiency as defined by NRES resolution. %SAT receptive fields.
    %


%
%**********************************************************************************************************************
%
%\section{Navigation by synthetic agents}
%\label{sec:navigation_by_AI}
%    Arguably the only system capable of autonomous navigation is the central nervous system of animalia;
%        Human, mammal, birds, and even insects are capable of autonomous navigation never possible in technology.
%    %Despite impressive accomplishments in machine learning and artificial intelligence, few examples exist of successful navigation or learning robotics based on AI.
%    %  Biological systems, however, learn by parallel processes in a massively distributed network with adaptive connections, allowing the necessary learning efficiency for real-world navigation.
%    We have seen how individual features can be expressed distributed across many feature detectors of one Euclidean space in the brain.
%    Further, biological computation is known to learn by parallel processes in a massively distributed network with adaptive connections, allowing the necessary learning efficiency for real-time navigation.
%    We will in this section explore to what degree a similar mechanism could be plausible in synthetic intelligence by our definition of SAT combined with reinforcement learning from AI.
%    %We will in this section explore how a similar mechanism could be accomplished by the concept of SAT combined with reinforcement learning (RL) from AI.
%
%%     In this text, we have seen several examples of distributed coding of SAT for navigation. %that is considered pertinent for navigation have been presented.
%%     % Distributed coding of SAT for several pertinent parameters for navigation have been discussed from the neuroscience literature.
%%     Examples from neural representation includes representation of own 
%%         location \cite{o1971hippocampus}, 
%%         head-direction \cite{taube1990head}, 
%%         borders \cite{solstad2008:border_cells} and boundaries \cite{lever2009boundary}, 
%%         and objects of interest \cite{deshmukh2013influence, hoydal2019object} have been discussed.
%%     A characteristic mechanism in all these representations is that individual cells represent Euclidean conditionals, allowing for population patterns that represent the current state of the agent.
%%     It has been reported that dead-reconing and other methods in navigation is possible due to grid cells being organized into discrete modules, where each module contains SAT with the same receptive field
%%         \ \cite{stemmler2015connecting}.
%%     From a computational point of view, such networks would be said to represent one-hot coding of the corresponding navigational parameter.
%%     %%%
%%     %The pattern of populations of neurons across all groups of NRES neurons combined can be said to represent the current state of the agent.
%%     %%
%%     %%Dette er kanskje en forklaring paa kvifor neurale sys. funker..
%
%
%    Knowledge of the geometric state of the environment can be referred to as orientation,
%    planning and acting according to this information could be referred to as navigation;
%        How can knowledge of navigational state be translated to active decisions based on experience?
%    First, for complex environments, adaptive orientation and navigation requires learning.
%    % TODO Skrive ut litt om RL. TODO :
%    The branch of machine learning able to learn to act based on earlier experience is referred to as \emph{reinforcement learning} (RL) in AI.
%    RL allows for adaptive behavior based on earlier experience\ \cite{sutton2018reinforcement}. 
%        Secondly, adaptive behavior needs to happen with such an efficiency that the result of learning can be seen real-time;
%    Active navigation should not be a result of analysis of large bodies of data as done in machine learning and statistical analysis.
%    % Deep learning and other statistical parameter search have proven to be difficult 
%    Real-world navigation does not have the luxury of speeding up computation and amounts of information that makes statistical analysis beneficial.
%
%
%    \begin{figure}[th!bp]
%        \centering
%        %\includegraphics[width=0.5\textwidth]{figures/gridworld}
%        \caption{The grid-world is a classic introductory example for reinforcement learning (RL).
%            \small
%            The agent accumulates experience during its lifespan; Every state-action pair that is visited causes an update of the Quality of doing that action from that state.
%            This is referred to as Q-learning\ \cite{sutton2018reinforcement}. % Obs: fig er ikkje derfra!
%            Tabular Q-learning is known to be limited with regards to the size of the state set, and is not used in robotics or navigation.
%        }
%        \label{fig:simple_GW}
%    \end{figure}
%    
%    We have seen how Euclidean spaces are represented in the biological brain:
%    Different considerations for navigational state are represented in populations of neurons, each node working as a feature detector of a SAT.
%    % A comprehensive coverage of the parameter set allows for a distributed coding of this aspect of navigational state.
%    Individual features, i.e.\ the conditional expressed through the receptive field for the SAT, could in this context be seen as the states that make up an RL challenge.
%    %Inspired by the learning efficacy of neural navigation, we define the state set as in a single NRES set.
%    The SAT interpretation of NRES, where individual features are represented by feature detectors, could form sets of SAT that represent mutually exclusive receptive fields.
%    
%    Every SAT of one particular NRES could further establish a separate learning challenge similar to the one shown in fig. \ref{fig:simple_GW}.
%    % These ideas, inspired by the\ \cite{stemmler2015connecting}, would be difficult to verify experimentally in biology as it would require knowledge of how all neurons of a population are connected. 
%    This could be done in layers, where each layer have the same lattice scale for all SAT, in addition to receptive fields of all containing SAT are non-overlapping (mutually exclusive).
%    For all experiments on this layout, we use the Karpathy WaterWorld learning environment\ \cite{webWaterWorldUnsolved_openai}.
%    WaterWorld represents a challenging task where the agent needs to avoid certain objects (red objects, reward -1) while catching others (green objects, reward +1).
%    %A full explanation of this simulation can be read under the comment section of the video-file of the simulation \cite{peerlearning_video}.
%    By the many individual learning challenges, each learning the policy toward accomplishing a single SAT, we can let the objects-of-interest define the priority of the resulting policy.
%    Let further policy be accumulated across across all relevant learners, in our attempt to replicate the distributed mechanism of neural navigation.
%
%    %An agent with a single NRES resolution layer is presented in figure \ref{fig:peerlearning_single_resolution:N5}.
%    %[left] An illustration of the setup of a single SAT layer, and [right] the accumulated score of a single run of this agent.
%    %The navigational AI shows promise in this challenging learning environment\footnote{According to openAI, this task is ``unsolved'' \cite{webWaterWorldUnsolved_openai}} RL task
%    \begin{figure}[th!bp]
%        \begin{minipage}[b]{0.34\textwidth}
%          %\includegraphics[width=\textwidth]{figures/bluedot_N5_with_elements_of_interest}
%          \vspace{3px}
%        \end{minipage}
%        \hfill
%        \begin{minipage}[b]{0.67\textwidth}
%          %\includegraphics[width=\textwidth]{figures/monoshepherd_accumulated_score}
%        \end{minipage}
%        \caption{A distributed approach to RL by NRES; Each of the SAT, represented as tiles in the illustration [left] represents a separate RL challenge.
%            Green and red crosses represent desirable and avoidable objects of interest. All information is represented in an allocentric reference frame.
%        [Right] The accumulated score for mono-layered NRES of different resolutions.}
%        \label{fig:peerlearning_single_resolution:N5}
%    \end{figure}
%
%    % Inspired by the sparse and distributed neural coding, I have implemented a simple navigational AI to handle an unsolved problem in reinforcement learning.
%    % A fundamental mechanism in neural computation, known as sparse coding, dictates that that input from several sources is combined to create the full picture.
%    In section \ref{sec:NRES_feature_extraction}, we have seen how NRES could be represented by discrete layers of SAT with the same resolution.
%    % In the hippocampal formation, we have seen NRES could be represented by discrete layers of SAT with the same 
%    % For each NRES of the navigational parameters in the hippocampal formation, evidence suggest that NRES is represented in layers of SAT with different resolutions.
%    Thinking of each tile in each layer as a separate challenge similar to the experiment from fig. \ref{fig:peerlearning_single_resolution:N5}, 
%        the agent could further be extended across multiple layers.
%    % This is beneficial from a functional point of view, as such a layout would enable the agent to quickly learn fundamental control but later be allowed to learn to a higher proficiency.
%    In the second experiment, we test the effect of implementing multiple layers with discrete lattice scale with regards to learning efficiency.
%    A layout inspired by the increasing resolutions along the dorsal-to-ventral axis of the hippocampus is illustrated in fig. \ref{fig:peerlearning_multi_resolution}.
%    To the right, we see the effect of combining multiple resolutions for navigation learning: 
%    %the results are promising, as the combination of {$N3$, $N7$, $N23$} attains more reward than the algebraic sum of its parts (the 3 mono-layered agents).
%        the results are promising, demonstrating the effect of combining orientational state across multiple resolutions.
%    \begin{figure}[th!bp]
%        \begin{minipage}[b]{0.5\textwidth}
%          %\includegraphics[width=\textwidth]{figures/illustrasjon_multi_shepherd}
%          \vspace{3px}
%        \end{minipage}
%        \hfill
%        \begin{minipage}[b]{0.5\textwidth}
%          %\includegraphics[width=\textwidth]{figures/interdimensional_peer_learning}
%        \end{minipage}
%        \caption{The distributed approach to RL by NRES can easily be extended to include multiple resolutions; Each SAT represented as tiles in the illustration [left] represents a separate RL challenge.
%            Three layers with mutually exclusive SAT are made, with resolution $N3$ (3X3 tiles), $N7$, and $N23$.
%        [Right] The accumulated score for multi-layered NRES performs better than the sum of its parts.}
%        \label{fig:peerlearning_multi_resolution}
%    \end{figure}
%        %[fig: peerlearning multi-layer]   [og: til høgre: vise resultat fra kjøringa!]
%
%    %The superposition principle 
%    The distributed approach from neural computation could further allows extending the orientation data set for navigation learning across multiple NRES.
%    % Superposition of multiple considerations are possible;
%    In the third experiment, we test the effect of adding NRES similar to the object-vector cells on top of the place cell NRES for navigation.
%    %The current heading (SAT similar to the one in head-direction cells) is used as the current parameter, with the objective set by the relative location of objects-of-interest.
%    Since sub-challenges are based on individual SAT, and each layer of NRES are learning in parallel, additional layers should not degrade learning performance.
%    %%
%    %We try an NRES that is perpendicular to the information expressed by place cells in experiments up till now;
%    We create an NRES inspired by Object-Vector Cells, where the agent learns to achieve the relative allocentric SAT of object-of-interest.
%    The new NRES information can be thought of as a combination of current heading, analogous to the head direction cell, and a relative allocentric SAT inspired by the object vector cell.
%    % Motivation and desire is still controlled by the reward received when some objective is acquired, and all aspects of the agent is now implemented under the SAT framework.
%    The immediate proficiency at the task can be seen in fig.\ \ref{fig:full_pupp} and in the video \cite{peerlearning_video};
%        Superposition of policy from multiple NRES can easily be extended, creating increasingly powerful navigational autonomy. %, without having to train for ages.
%    Since individual layers are trained separately, in full parallel, this effect is achieved without increasing the learning time for the agent 
%        (compare the transient part of the curves in fig. \ref{fig:full_pupp}).
%    %  We have seen that this can be done without significantly increasing training times, making real-world navigational autonomy plausible.
%
%
%    %We could define the self state as a combination of representation HDC + speed cell for current state, plus OVC for objectives.
%    %The distributed computational approach assimilated from neuroscience allows for these to exist alongside each of the SAT from experiment 2 (fig>peerlearning, multilayer,results(HS)).
%    \begin{figure}[th!bp]
%        %\includegraphics[width=\textwidth]{figures/interdimensional_peer_learning_multiparameter}
%        \caption{
%            Navigation by a orientational state as expressed by distributed NRES allows for learning by superposition of input. %can be extended without increasing training time.
%            %The distributed approach to RL by NRES can easily be extended to include multiple NRES;
%            Place cell SAT is listed as \emph{Position}. 
%            % and ``object vector cell + head direction'' is referred to as \emph{Speed} (since heading and relative displacement measured from the current speed vector).
%            Heading and relative displacement measured from the current speed vector is reported by \emph{Speed}.
%            This is inspired by the combination of the SAT of object vector cell with information of head direction.
%            Note that the data from \emph{Multi-Feature Position} is equivalent to the best result from fig. \ref{fig:peerlearning_multi_resolution}.
%                %that \emph{Multi-Feature Speed} learns better, but the combination achieves a higher final proficiency, faster, than its components combined.
%            %The computational load of the system, a normal limitation in AI, scales linearly with the highest resolution, not the number of layers. 
%            %Traditional RL is infamous for having an exponential increase in learning time with the number of states. \\
%            %This result is promising with regards to allowing for autonomous navigation.
%        }
%            \label{fig:full_pupp}
%    \end{figure}
%}}}

